World-set Decompositions: Expressiveness and Efficient Algorithms

Uncertain information is commonplace in real-world data management scenarios. The ability to represent large sets of possible instances (worlds) while supporting efficient storage and processing is an important challenge in this context. The recent formalism of world-set decompositions (WSDs) provides a space-efficient representation for uncertain data that also supports scalable processing. WSDs are complete for finite world-sets in that they can represent any finite set of possible worlds. For possibly infinite world-sets, we show that a natural generalization of WSDs precisely captures the expressive power of c-tables. We then show that several important decision problems are efficiently solvable on WSDs while they are NP-hard on c-tables. Finally, we give a polynomial-time algorithm for factorizing WSDs, i.e. an efficient algorithm for minimizing such representations.

==> revision-note <==
Dear Reviewers

Many thanks for the very helpful comments of the two reviewers.  Their
comments definitely led to clear improvements of our article. We
considered all of them. Below are our comments on how we improved the
article.

------------------------------------------------------------------
Comments for Reviewer 1.

- Table 2: Please change "pos relational algebra" by "positive
relational algebra".

Response: done.


- After Example 1: It would be a good idea to add an example of a
c-table showing how local conditions are used (and why they are
important for c-tables).

We added Example 1 that comments on two c-tables used throughout the article 
(from Sec 1 and Fig 6(a)).

- After Definition 2: Please add a note saying why condition (3) is
important in Definition 2. In particular, you should say that this
definition makes sense even if the infinite domain D and the set of
natural numbers N are disjoint, since the conditions in M(Y,\mu) are
used to select tuples from T (instead of specifying what are the
possible values in the cells of the relations in rep(T), which is done
by using conditions of the form $x = c$, $y \neq d$, ..., where c and
d are in D).

Response: We added an example (Example 3) discussing two x-multitables
and how mutex conditions are used. We hope that this improvement helps
the reader understands faster and easier the main ideas behind
x-multitables.


- Proposition 3: Please say that the query is considered to be fixed
in the polynomial time result (data complexity).

Response: done.


- The definition of function rep for gWSDs is confusing. Assume that R
is a relation with attributes A_1, ..., A_k. Then in every tuple of
a gTST, we have that R.d_i.A_1, .., R.d_i.A_k are either all different
from \bot or all equal to \bot. For example, Figure 3 (b) shows a gTST
satisfying this condition, while the following table does not satisfy
this condition:

     |  R.d_1.A_1  R.d_1.A_2 
----------------------------
     |     5          6
     |     7         \bot


At the beginning of Section 3.2, a gWSD ({C_1, ..., C_n}, \phi) is
defined as an m-decomposition of a gTST (W, phi), that is, W  = C_1
\times ... \times C_n, and function rep for gWSDs is defined as:

rep({C_1, ..., C_n}, \phi) = rep(C_1 \times ... \times C_n, \phi).

This definition only considers the case where C_1, ..., C_n is an
m-decomposition of some gTST. What happens if this is not the case? In
particular, what happens if the product C_1 \times ... \times C_n does
not satisfy the condition mentioned above (that is, there is a tuple
in the product where some R.d_i.A_j has value \bot and some R.d_i.A_k
has value different from \bot)? For example, C_1 \times C_2 does not
satisfy the condition mentioned above if C_1 and C_2 are the following
tables:


C_1  |  R.d_1.A  R.d_1.B 
----------------------------
     |     1        2
     |     3        4


C_2  |  R.d_2.A  R.d_2.B 
----------------------------
     |     5        6
     |     7       \bot

In this case, how do you define function rep for C_1 \times C_2? This
is an important point in the proof of NP-hardness in Theorem 1. In
fact, from this proof and footnote 7, the reader can infer that in the
previous example, tuple (7, \bot) is equivalent to (\bot, \bot). The
authors should clarify this point, and they should define the function
rep for the general case (not only for a gWSD that corresponds to an
m-decomposition of some gTST). 


Response: This is a very helpful observation. We now see that the
problem already occurs when defining gTSTs. We decided to allow
several possible inlining functions of g-tabsets into gTSTs (see page
10): a valid inlining does not need to add only \bot symbols for the
missing values, but also arbitrary values or variables such that a
"dummy" added tuple has at least one \bot-value. All such "dummy"
tuples are equivalent to the tuple that only has \bot
values. Arbitrary gWSDs, as the one given by the reviewer, can now be
obtained by decomposing an appropriate gTST.


- Corollary 1 and Proposition 7: At a first glance, these two results
are confusing since vWSDs are more expressive than WSDs. In fact,
Corollary 1 is a consequence of Proposition 6 and the fact that
every WSD represents a finite set of possible worlds, which is not the
case for vWSDs. Please say this after Corollary 1.

Response: added an explanation between Corollary 1 and Proposition 7
to point out that in the case of infinite world-sets vWSDs are weaker
than WSDs in the finite case.


- Proof of Proposition 7: When you assume that T has a single tuple of
the form <A:1, B:x>, you should say that T represents the world <A:1,
B:1> since in a v-tabset, the global condition is a conjunction of
equalities and, thus, you cannot use the condition $x \neq 1$.

In this proof, change tuple <1,z> by <A:1, B:z>.

Response: we rephrased this proof and hope it is more understandable
now. We also use now consistently the tuple notation noted by the
reviewer.


- Proof of Theorem 1: Give the definition of Exact Cover by 3-Sets (X3C).

Also, it would be a good idea to move the last paragraph ("It follows
that the problem of deciding ...") outside the proof. You can put it
before Corollary 2.

Response: done (both).


- Example 3: Explain why WSD {C_1, C_2, C_3} represents the empty
world (every tuple d_i has the symbol \bot in some attribute in the
result of combining the first tuple in C_1, the third tuple in C_2 and
the fourth tuple in C_3).

Response: the suggested explanation was added.

- Proof of Lemma 1: $n_j$ is used before being defined (number of
tuples in C_j). Also, please change c-multitable by x-multitable
everywhere. 

Response: we re-wrote the proof of Lemma 1. We use the same
construction, but rephrased the correctness proof to make it clearer.

Also in this proof, it would be a good idea to add a note explaining
why when n_j > 1, you use constraint x_j = i for i < n_j and
constraint (x_j \neq 1 \wedge ... \wedge x_j \neq n_j-1) for i =
n_j. To make the proof more clear, you could move Example 4 inside the
proof (you could put this example before the proof of correctness). In
this example, you can explain why you have to consider two different
types of constraints for n_j > 1 (you could say that if you replace
$x_1 \neq 1$ by something like $x_1 = 2$ in the example, then when
$x_1$ gets assigned value 3, you do not obtain any tuple and, thus,
the x-table could not represent the 1-gWSD in Figure 5 (a)).

Response: we inlined our example (now Example 6) in the proof and also
explain the cases mentioned by the reviewer.


- Proof of Lemma 2: Please say that you can assume, without loss of
generality, that all the variables in a c-table are different since if
you have the same variable x in two different positions, then you can
replace one occurrence of x by y and then add the conjunct x = y to
the global condition.

Response: we re-wrote this proof and hope it is clearer now. we
realized that it is more natural to translate c-multitables into
g-tabsets (using the set of consistent \Theta's from the previous
version of the proof). We then re-use existing results on inlining
g-tabsets into gTSTs, which are in fact 1-gWSDs.

In this proof, you say that you compute "a set of consistent \Theta
...". Maybe i am missing something, but from the proof of (1), the
reader can infer that you need "the set of all consistent \Theta ...".
Please clarify this point.

Response: yes, we need the set of all consistent \Theta's.


- Example 5: Please explain how you obtain the 1-gWSD in Figure 6 (b)
from the c-table T in Figure 6 (a) (what are the sets \Theta used in
this construction?)

Response: We added the \Theta's used in the construction, see Fig 6
and Example 7.

- Section 5: In this section, you talk about the q-possibility problem,
while in the introduction you talk about the $Q$-possibility
problem. Please use only one name for this problem (same for q-certainty,
...).

Response: we now use "q" instead of "Q" everywhere.


- Proof of Theorem 4: It is clear that the problem of deciding whether
\bigwedge_i c_i is satisfiable is equivalent to deciding whether there
is a world A where the answer to S - R is empty, but since in this
theorem you are proving the NP-hardness of tuple q-possibility for full
relational algebra, please change the previous equivalence by
something like: the problem of deciding whether \bigwedge_i c_i is
satisfiable is equivalent to deciding whether there is a world A where
$t \in Q(A)$, where $Q$ and $t$ are defined as ..., and then prove
this equivalence.

Response: very good point :-) In that version, the proof shows
instance q-possibility and not tuple q-possibility. We did a minor
tweak to solve the problem and now check for the nullary tuple to be
possible in the answer to {<>} - \pi_{\emptyset}(S-R). That is, the
nullary tuple is in the answer precisely when S-R is empty.


- After proof of Theorem 5: Please add a paragraph explaining why
tuple possibility and certainty are difficult to solve on c-tables
(you should emphasize here that one of the advantages of gWSDs is that
these two problems can be solved efficiently).

Response: We added a comment on this after Th 5 (tuple possibility).

- Proof of Theorem 9: In the first two lines, "positive relational
algebra" should be replaced by "full relational algebra".

Response: done.

- First paragraph of Section 6: The authors claim that the algorithm
presented in this section can compute "good" non-optimal
factorizations of gWSDs (by treating variables as constants). The
authors do not explain why they claim this. In fact, they do not
provide any criteria for evaluating the quality of the results of the
algorithm for gWSDs. The authors should clarify this point.

Response: we dropped that (unfounded) remark. We also moved the
discussion on how relational factorization can be used for gWSD
optimization in Sec 6.3 (where we also formalize our statement that
tuple-level WSDs have unique maximal decompositions).


------------------------------------------------------------------
Comments for Reviewer #2.

1. Provide examples before formal definitions - that will make the article much more
readable.

Response: we added several new examples (Ex 1, 3; Fig 12 & 13) and
improved existing ones (now Ex 5, 6, 7, 8).

2. Organize section 5 into one subsection per complexity result to make the section
more readable.

Response: We organized Sec 5 into the subsections consisting of
theorems that are somehow connected. For instance, the theorem for
tuple possibility is obtained immediately from tuple q-possibility and
we therefore decided to group them together.

3. At the beginning of each section, include a few lines explaining the flow in
sections eg. in section 2 (provide the list of important definitions in the section
up front and indicate how they will be used in the rest of the article),

Response: We did this for Sec 2.1, 3, and 6. Sec 4 and 5 already had
such introductions.

4. It would be a good idea to summarize the relationships (expressive power,
'succintness' etc) between the different types of tables (c,g,v-multitables,
cgv-tables, mutex tables) and representation systems (c,g,v-tabset,
c,g,v-tabset-table, c,g,v-WSD {attribute-level and tuple level}. I had to sketch an
illustration myself in order to better understand the concepts.

Response: We sketched the known relationships between the expressive
power of tuple-level formalisms at the end of Sec 4 (after Corollary
4). We also added that gWSDs are more expressive than vWSDs (using the
results on the weakness of vWSDs). Succinctness of g(v)WSDs over
g(v)TSTs (and thus over tabsets) and is now emphasized in Sec 3.2
after Remark 3, Proposition 8, and Dfinition 5.



Specific comments:
1. Provide a brief explanation of what is different in the extended version as
compared to the original paper [6].

Response: see footnote 3.

2. Page 4 (line 3): describe briefly what v-tables are to aid the reader, provide a
reference here in addition to the reference in Table 2 for v-tables

Response: we added an additional reference to v-tables; they are
explained in point 2 after Proposition 1.

3. Page 4 (line 4 from the end): show where in the article you show that gWSDs are
strictly stronger than Trio. Also, indicate what you mean by 'strictly stronger'.

Response: we inlined the explanation for our statement: Trio can only
represent finite world-sets, whereas gWSDs can represent infinite
world-sets (in addition to all finite world-set).

4. Section 2.1: Provide examples for {c,v}-multitables, mutex-set. 

Response: added Example 1 for c-multitables and Example 3 for
x-multitables and mutex sets.

5. Page 7, line 2: typo - 'negated qualities' should be 'negated equalities'

Response: corrected.

6. Page 7, last line: An example would definitely help to better understand mu in
mutex tables.

Response: we added Example 3 and we also explain mutex sets later in
Example 6 (now inlined in the proof of Lemma 1).

7. Section 3.2, Page 11, line 6: 'Clearly, A and any gWSD of A...' - what is A?
g-tabset? Make it more explicit.

Response: done.

8. Section 3.2, Page 11, Proof of Proposition 7: 'Let T = {T_1,..., T_n} ... over
schema (R_1,..., R_m)...'. Are you indicating that the number of tables and schemas
are different (n vs m)?

Response: we changed that notation. We wanted to state that there is
no constraint on n versus m (they can be different or equal).

9. Section 4, Page 15, Construction section of Lemma 1: what is n_j? what are w_i's?
Make them explicit.

Response: the proof was improved and the notation is made explicit.

10. Section 4, Page 15, Construction section of Lemma 1: Can rewrite 'which encodes
to which row of component C_j a tuple belongs to' as 'which encodes the row of
component C_j to which a tuple belongs'.

Response: we rephrased the whole proof, including that sentence.

11. Section 4, Page 15: Indent 'Correctness' section to the same level as
Construction section.

Response: done.

12. Page 23, Theorem 9, construction section: typo: 'Q := ... (R.r_1 X R.r_2 X
R.r_3), where'

Response: we rewrote Q to ..( (R r_1) X (R r_2) x (R r_3)).







